Incremental Randomized Smoothing Certification

Randomized smoothing-based certification is an effective approach for obtaining robustness certificates of deep neural networks (DNNs) against adversarial attacks. This method constructs a smoothed DNN model and certifies its robustness through statistical sampling, but it is computationally expensive, especially when certifying with a large number of samples. Furthermore, when the smoothed model is modified (e.g., quantized or pruned), certification guarantees may not hold for the modified DNN, and recertifying from scratch can be prohibitively expensive. We present the first approach for incremental robustness certification for randomized smoothing, IRS. We show how to reuse the certification guarantees for the original smoothed model to certify an approximated model with very few samples. IRS significantly reduces the computational cost of certifying modified DNNs while maintaining strong robustness guarantees. We experimentally demonstrate the effectiveness of our approach, showing up to 3x certification speedup over the certification that applies randomized smoothing of the approximate model from scratch.

==> intro-old.tex <==
Deploying and optimizing Deep Neural Networks (DNNs) on real-world systems with bounded computing resources (e.g., edge devices), have led to various techniques for approximating DNNs while maintaining high accuracy and robustness. 
Common approximation techniques are quantization -- reducing the numerical precision of weights~\citep{zhou2017incremental}, and pruning -- removing weights that have minimal impact on accuracy~\citep{DBLP:conf/iclr/FrankleC19}.


For trustworthy deployment of DNNs, randomized smoothing (RS) is a promising approach for obtaining robustness certificates by constructing a smoothed model $g$ from a base network $f$ under noise~\cite{DBLP:conf/icml/CohenRK19}. 
%
To certify the model $g$ on an input, RS certification checks if the estimated lower bound on the probability of the top class is greater than the upper bound on the probability of the runner-up class (with high confidence).
%
\add{ RS certification computes the certified accuracy metric of the DNN on the set of test inputs as a proxy for the DNN robustness.


Despite its effectiveness, RS-based certification can be computationally expensive as it requires DNN inference on a large number of corruptions per input. 
%
For instance, certifying a quantized ResNet-50 network on only 500 images from the ImageNet test dataset takes more than 50 hours on a device with a CPU (Section~\ref{sec:exp_quant}).
%
When a user seeks to select an accurate and robust network from a range of possible approximate networks \cite{10.5555/3291168.3291211, 10.5555/3327144.3327258, 10.1145/3360612}, each approximate network needs to be certified.
%
Although the approximate DNNs are obtained by slight perturbations in the DNN weights and have largely similar behavior, RS certification needs to be performed from scratch since guarantees do not transfer across networks. 
%
The existing RS certification process often consumes substantial time in this setting due to the multitude of network choices.
% Previous research leveraged RS to certify the robustness of approximate models, e.g.~\citep{voracek2023sound, DBLP:conf/iccv/Lin00S21} for quantization and~\citep{sehwag2020hydra} for pruning.
%

% \fTBD{Why would we ever certify in low-end device when you can do that on workstaton, like you did here?}
% Moreover, when a user seeks to select an approximate network from a range of possibilities \cite{10.5555/3291168.3291211, 10.5555/3327144.3327258, 10.1145/3360612}, the certification process often consumes substantial time due to the multitude of network choices and we need to run certification from scratch for each network.

 % Moreover, in the context of approximation tuning, the user seeks to select an approximate network from a range of possibilities with different approximation choices for each network layer \cite{10.5555/3291168.3291211, 10.5555/3327144.3327258, 10.1145/3360612}.  The tuning should ensure a minimum user-defined metric such as certified accuracy. This tuning process often consumes substantial time due to the multitude of network choices and we need to run certification from scratch for each new network with existing approaches. 

This underscores a major limitation of almost all existing RS-based certification techniques in the above setting, that the certification needs to be run from scratch every time the network is even slightly modified. Overcoming this main limitation requires addressing a fundamental problem:

\vspace{.06in}
\noindent{\fbox{\parbox{\dimexpr\linewidth-2\fboxsep-2\fboxrule\relax}{Can we leverage the information generated while certifying a given network to speed up the certification of its approximate versions?}}}
\vspace{.03in}


\paragraph{This Work.} We present the first incremental RS-based certification framework called Incremental Randomized Smoothing (\Tool{}) to address these challenges. The primary objective of our work is to improve the sample complexity of the certification process of approximate networks on a predefined test set. Improved sample complexity results in overall speedup in certification, and it reduces the energy requirement and memory footprint of the certification. Given an original network $f$ and its smoothed version $g$, and a modified network $f^p$ with its smoothed version $g^p$, \Tool{} incrementally certifies the robustness of $g^p$ by reusing the information from the execution of RS certification on $g$. }
%
% The motivation of the IRS, similar to many existing incremental techniques in program breakdown \cite{Lachnech-etal:TACAS01, DBLP:conf/lics/OHearn18} and more recently deterministic DNN certification ~\citep{DBLP:journals/pacmpl/UgareSM22, DBLP:journals/corr/abs-2106-12732, ugare2023incremental}, is not certifying a single network from scratch. It is applicable when certifying multiple similar networks. Where, it can reuse the certification of one of the networks, for faster certification of all other similar networks.


% Despite its effectiveness, RS-based certification can be computationally expensive as it requires DNN inference on a large number of input corruptions. 
% In particular, when the base classifier $f$ is approximated to $f^p$, the certification guarantees do not hold for the new smoothed classifier $g^p$, and certifying $g^p$ from scratch can be expensive. 

% % Incremental verification paragraph and why it not enough 
% To improve the efficiency of the certification of $g^p$ one can \emph{incrementally} certify it by reusing the parts of certification of $g$. 
% Indeed, recent works have developed incremental certification techniques based on formal logic reasoning~\citep{DBLP:journals/pacmpl/UgareSM22, DBLP:journals/corr/abs-2106-12732, ugare2023incremental} for improving the certification efficiency of $f^p$ by reusing the certification of $f$. 
% However, these techniques perform incremental \emph{deterministic} certification that cannot scale to high-dimensional inputs e.g., ImageNet, or state-of-the-art models, e.g. ResNet (their evaluation demonstrated effectiveness only for small CNNs, up to 8-layer, on CIFAR10). To support state-of-the-art models and datasets, we instead need to think of a new scalable framework that can incrementally speed up \emph{probabilistic} methods like RS.


% \paragraph{This Work.} We present the first incremental RS-based certification framework called Incremental Randomized Smoothing (\Tool{}) to address these challenges. Given an original network $f$ and its smoothed version $g$, and a modified network $f^p$ with its smoothed version $g^p$, \Tool{} incrementally certifies the robustness of $g^p$ by reusing the information from the execution of RS certification on $g$.

% Our approach makes 3 key insights This is our algo and how it works
% When certifying robustness around input $x$ on a smoothed classifier $g$ using RS, lower and upper bounds ($\palb$ and $\pbub$) are estimated for the probabilities of the top-class $A$ and the "runner-up" class $B$ respectively. 
% The certified radius is then calculated as $\frac{\sigma}{2} (\Phi^{-1}(\palb) - \Phi^{-1}(\pbub))$.

% For certifying the smoothed classifier $g^p$, \Tool{} optimizes the process by computing the similarity estimation $\eqlb$ between $f$ and $f^p$. 
% Our insights: (1) Common approximations yield smaller $\eqlb$ values, (2) Estimating $\eqlb$ through binomial confidence interval requires fewer samples as it is close to 0, and (3) $\eqlb$ can be leveraged alongside precomputed $\palb$ and $\pbub$ values from $f$ to compute the certified radius as $\frac{\sigma}{2} (\Phi^{-1}(\palb-\eqlb) - \Phi^{-1}(\pbub+\eqlb))$ for $g^p$. 

\Tool{} optimizes the process of certifying the robustness of smoothed classifier $g^p$ on an input $x$, by estimating \emph{the disparity} $\eqlb$ -- the upper bound on the probability that outputs of $f$ and $f^p$ are distinct. 
%
Our new algorithm is based on three key insights about disparity:

\vspace{-.05in}
\begin{enumerate}\itemsep 1pt\parskip 2pt
\item Common approximations yield small $\eqlb$ values -- for instance, it is below 0.01 for int8 quantization for multiple large networks in our experiments. 
\item Estimating $\eqlb$ through binomial confidence interval requires fewer samples as it is close to 0 -- it is, therefore, less expensive to certify with this probability than directly working with lower and upper probability bounds in the original RS algorithm.
\item We can leverage $\eqlb$ alongside the bounds in the certified radius of $g$ around $x$ to compute the certified radius for $g^p$ -- thus soundly reusing the samples from certifying the original model.
%
\end{enumerate}
%\Tool{} enhances certification efficiency by leveraging these insights for estimating $\eqlb$ and reusing previous bounds to compute the certified radius for updated smoothed classifier $g^p$.

\vspace{-.05in}
We extensively evaluate the performance of \Tool{} on state-of-the-art models on CIFAR10 (ResNet-20, ResNet-110) and ImageNet (ResNet-50) datasets, considering several common approximations such as pruning and quantization. Our results demonstrate speedups of up to \upto over the standard non-incremental RS baseline, highlighting the effectiveness of \Tool{} in improving certification efficiency. 

\paragraph{\bf Contributions.} The main {contributions} of this paper are:
% One more about the concept of incremental RS

\vspace{-.15in}
\begin{itemize}\itemsep 1pt \parskip 2pt
    \item We propose a novel concept of incremental RS certification of the robustness of the updated smoothed classifier by reusing the certification guarantees for the original smoothed classifier. 
    \item We design the first algorithm \Tool{} for incremental RS that efficiently computes the certified radius of the updated smoothed classifier. 
    \item  We present an extensive evaluation of the performance of \Tool{} speedups of up to \upto over the standard non-incremental RS baseline on 
    state-of-the-art classification models. 
\end{itemize}


% \vspace{-0.1in}
% \noindent \Tool{} code is available at {\color{blue}\url{https://github.com/uiuc-arc/Incremental-DNN-Verification}}.
% \vspace{-0.15in}


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tables/t2.tex <==
%---------------
\begin{table}[ht]
    \small
    \centering
    \caption{Average \Tool{} certification accuracy speedup for combinations of radius, quantizations, and $\sigma$'s on ImageNet ResNet-50.}
    \begin{tabular}{@{}ll rrr@{}}
        \toprule
        $\sigma$ & Radius & \multicolumn{3}{c}{Quantization} \\
        & & fp16 & bf16 & int8 \\
        \hline
        & 0.25 & 3.92x & 1.85x & 3.61x \\
        0.5 & 0.5 & 2.7x & 1.6x & 2.67x \\
        & 0.75 & 1.2x & 1.12x & 1.23x \\
        \hline
        & 0.5 & 4.79x & 3.07x & 4.44x \\
        1.0 & 1.0 & 2.6x & 2.25x & 2.6x \\
        & 1.5 & 1.53x & 1.38x & 1.54x \\
        \hline
        & 1.0 & 5.3x & 3.31x & 4.06x \\
        2.0 & 2.0 & 2.79x & 2.46x & 3.94x \\
        & 3.0 & 1.51x & 1.48x & 1.80x \\
        \bottomrule
    \end{tabular}
    \label{tab:avg_acc_speedup}
\end{table}

%----------------------

==> tables/t_end2end.tex <==
%---------------
\begin{wraptable}{r}{.55\textwidth} 
    \tablesize
    \centering
    \vspace{-0.15in}
    \caption{\Tool{} end-to-end speedup for ResNet-110 on CIFAR-10 and ResNet-50 on ImageNet with $\sigma$ = 1.}
    \begin{tabular}{@{}lll rrr@{}}
        \toprule
        Dataset & Architecture & \#Networks & speedup\\
        \hline
        & & 2 & 2.59x  \\
        CIFAR10 & ResNet-110  & 3 & 2.84x \\
        & & 4 & 3.00x \\
        \hline
         & & 2 & 1.29x \\
        ImageNet & ResNet-50 & 3 & 1.30x \\
        & & 4 & 1.31x \\
        \bottomrule
    \end{tabular}
    % \vspace{-0.4in}
    \label{tab:end2end}
\end{wraptable}

%----------------------

==> tables/t_reduction.tex <==
%---------------
\begin{wraptable}{r}{.55\textwidth} 
    \tablesize
    \centering
    \vspace{-0.15in}
    \caption{Time taken by \Tool{} and baseline for certifying int8 quantized .}
    \begin{tabular}{@{}lll rrr@{}}
        \toprule
        Dataset & Architecture & $ACR$ & $T_{\textit{base}}$ & $T_\textit{\Tool{}}$ &  $T_\textit{saved}$\\
        \hline
        CIFAR10 & ResNet-110 & 0.56 & 2.91h & 0.71h & 2.12h \\
        & & 0.85 & 15.39h & 11.32h & 4.07h \\
        ImageNet & ResNet-50 & 0.875 & 27.82h & 22.45h & 5.36h \\
        & & 0.90 & 53.93h & 40.58h & 13.35h \\
        \bottomrule
    \end{tabular}
    % \vspace{-0.4in}
    \label{tab:avg_speedup}
\end{wraptable}

%----------------------
